FiGURe: Simple and Efficient Unsupervised Node Representations with Filter Augmentations

Unsupervised node representations learnt using contrastive learning-based methods have shown good performance on downstream tasks. However, these methods rely on augmentations that mimic low-pass filters, limiting their performance on tasks requiring different eigen-spectrum parts. This paper presents a simple filter-based augmentation method to capture different parts of the eigen-spectrum. We show significant improvements using these augmentations. Further, we show that sharing the same weights across these different filter augmentations is possible, reducing the computational load. In addition, previous works have shown that good performance on downstream tasks requires high dimensional representations. Working with high dimensions increases the computations, especially when multiple augmentations are involved. We mitigate this problem and recover good performance through lower dimensional embeddings using simple random Fourier feature projections. Our method, FiGURe achieves an average gain of up to 4.4%, compared to the state-of-the-art unsupervised models, across all datasets in consideration, both homophilic and heterophilic. Our code can be found at: https://github.com/microsoft/figure.

==> sections/dump.tex <==
%%%%%%%%%%%%%%%%%%%% RQ1

% We present important observations from Table \ref{tab:main_table_results}. Across both homophilic and heterophilic datasets, we observe that \ourmethod~ outperforms the best unsupervised model in each case, except on \citeseer, \squirrel~ and \minesweeper~  where it achieves matches the best performance. Despite this highly competitive performance across the board, we want to emphasize that our actual value of interest lies in the rightmost column, which represents the average percentage gain in performance across the different datasets. In other words, for each model, the improvement that \ourmethod~ provides is calculated for each dataset, and this improvement is then averaged across all the datasets. The reason we report this number is to emphasize that despite some models seemingly having a percentage point advantage on specific datasets, no baseline is able to perform as consistently well across all the datasets as \ourmethod. Even the more recent state of the art contrastive models \grace~ and \sugrl~ suffer, on an average, by 5\% and 10\% respectively. Since \ourmethod~ is explicitly capturing information from different parts of the eigenspectrum, it as able to perform consistently well without making assumptions about the data. Therefore, \ourmethod is able to learn the most general and task agnostic representation. 

We analyzed the results presented in Table \ref{tab:main_table_results} and made several important observations. Firstly, across both homophilic and heterophilic datasets, \ourmethod~ consistently outperforms the best unsupervised model, except for a few specific cases where it achieves comparable performance. More importantly though, we want to draw attention to the rightmost column of the table, which represents the average percentage gain in performance across all datasets. This is calculated by comparing the improvement that \ourmethod~ provides over each baseline model for each individual dataset, and then averaging these improvements across all datasets. Using this metric, we highlight the overall performance consistency of \ourmethod~across diverse datasets. We found that no other baseline model achieves the same level of consistent performance across all datasets as \ourmethod. Even the more recent state-of-the-art contrastive models \grace~and \sugrl~experience average performance drops of $\sim$5\% and $\sim$10\%, respectively. This indicates that \ourmethod~is able to learn representations that are not only competitive on specific datasets but also exhibit high generalization and task-agnostic capabilities.


% Secondly, to demonstrate the applicability of RFF projections to improve lower dimensional representations we provide comparisons with \ourmethod at 32 and 128 dimensions (\ourmethod$_{32}$ and \ourmethod$_{128}$). Remarkably, using RFF, even at lower dimensions \ourmethod is able to provide competitive performance across datasets, beating the 512 dimensional baselines in several cases. Further insights about the effectiveness of RFF projections are revealed in RQ2.

Another important observation from our results is the applicability of RFF projections to improve lower dimensional representations. We conducted comparisons between \ourmethod~at different dimensions, including \ourmethod$_{32}$ and \ourmethod$_{128}$ which correspond to learning $32$ and $128$ dimensional embeddings respectively, in addition to the baseline representation size of 512 dimensions. Remarkably, even at lower dimensions, \ourmethod~with RFF projections demonstrates competitive performance across datasets, surpassing the 512-dimensional baselines in several cases. This highlights the effectiveness of RFF projections in enhancing the quality of lower dimensional representations. More insights about the effectiveness of RFF projections and their impact on performance are discussed in Section \ref{subsec:exp_rff_projections}.

% Additionally, to provide a benchmark for comparison, we also include the widely used supervised model, \gcn~in Table \ref{tab:gcn_table_results}. Despite being unsupervised, \ourmethod ~consistently outperforms \gcn~on heterophilic datasets, except for \romanempire~and \minesweeper, while achieving competitive performance on homophilic datasets. We provide further comparisons with supervised methods in the supplementary material. It is important to note here, that the motivation for learning using multiple filters comes from models like \gprgnn, which learn a task specific representation, by learning how to utilize information from different parts of the eigenspectrum effectively for the task at hand. We show, through the success of \ourmethod, that it is possible to learn these representations in an unsupervised and task agnostic manner. The only task specific part is how to combine these learned representation, using \todo a weighted sum combination in the downstream supervised task.

Furthermore, to establish a benchmark for comparison, we include the widely used supervised model, \gcn, in Table \ref{tab:gcn_table_results}. Notably, \ourmethod~ outperforms \gcn~on heterophilic datasets, with the exception of \romanempire~and \minesweeper, while achieving competitive performance on homophilic datasets. Detailed comparisons with supervised methods can be found in the supplementary material. It is important to highlight that the motivation for learning using multiple filters stems from models like \gprgnn, which aim to learn task-specific representations by effectively utilizing information from different parts of the eigenspectrum. In the case of \ourmethod, we demonstrate that it is possible to learn these representations in an unsupervised and task-agnostic manner. The only task-specific aspect lies in how these learned representations are combined, utilizing a weighted sum combination method (see \ref{subsec:supervised_representation_learning}) in the downstream supervised task.


%%%%%%%%%%%



RQ2



In this section, we will analyze the performance of unsupervised baselines by utilizing 32 and 128 dimensional embeddings and considering the presence or absence of RFF projections. Detailed insights into these comparisons can be found in Table \ref{tab:rff_table_32}. We would like to emphasize that, despite extensive hyperparameter tuning, we were unable to replicate the results reported by \sugrl. Therefore, we present the best results we were able to obtain. These tables yield two noteworthy observations.

Firstly, it becomes evident that meaningful and linearly separable representations can be derived from lower dimensional embeddings through the application of simple RFF projections. The inclusion of RFF projections consistently enhances performance in almost all cases. This finding strengthens the idea that existing Mutual Information-based methods can capture valuable information even when using lower-dimensional embeddings. Additionally, it emphasizes the effectiveness of RFF projections in improving the learned representations.


Secondly, it is evident that \ourmethod~consistently achieves superior or comparable performance compared to the baselines, even when operating in lower dimensions. Notably, this includes \sugrl, which is purported to excel in learning representations in such settings. However, there exists a 2-3 percent performance gap between \grace~and our method in the case of the \squirrel~and \chameleon~datasets. Although \grace~demonstrates proficiency in handling heterophily at lower dimensions, its performance significantly deteriorates when dealing with homophilic graphs. This indicates that, unlike \ourmethod, \grace~struggles to capture information of lower frequency, thereby limiting its effectiveness. Moreover, our method exhibits computational efficiency advantages on certain datasets when operating in lower dimensions. Further details about this can be found in the supplementary material.


Overall, the findings from RQ2 emphasize the potential of RFF projections in extracting useful information from lower dimensional embeddings and reaffirm the competitiveness of \ourmethod~ over the baselines.



\subsection{RQ3: Sharing Weights Across Filter Specific Encoders}
\label{subsec:enc_weight_sharing}
\begin{table}[ht]
    \small
    \renewcommand*{\arraystretch}{1.2}
    \centering
    \caption{A comparison of the performance on the downstream node classification task using independently trained encoders and weight sharing across encoders is shown in Table \ref{tab:independent_vs_shared}. The reported metric is accuracy, and a higher value indicates better performance. In both cases, the embeddings are combined using the same method as described in Section \ref{subsec:supervised_representation_learning}. $\Delta$ indicates the difference in accuracy between the shared encoder and independent encoder.}
    \begin{tabular}{ccccc}
    \hline
         & \cora & \citeseer & \squirrel & \chameleon \\ \hline
        \textsc{Independent} & 86.92 (1.10) $\%$ & 75.03 (1.75) $\%$ & 50.52 (1.51) $\%$ & 66.86 (1.85) $\%$ \\ 
        \textsc{Shared} & 87.00 (1.24) $\%$ & 74.77 (2.00) $\%$ & 52.23 (1.19) $\%$ & 68.55 (1.87) $\%$ \\ \hline
        $\Delta$  & \textbf{0.08} $\%$ & \textbf{-0.26} $\%$ & \textbf{1.71} $\%$ & \textbf{1.69} $\%$ \\ \hline
    \end{tabular}
\label{tab:independent_vs_shared}
\end{table}
To verify the claim that the computational load can be reduced by sharing the weights of the encoder across filters without sacrificing performance, we conducted the experiment presented in Table \ref{tab:independent_vs_shared}. In this experiment, independent encoders were trained on each filter individually, and the resulting embeddings were combined as described in Section \ref{subsec:supervised_representation_learning}, for the downstream node classification task. The performance of these independent encoders was then compared with the results obtained from the shared encoder (for the same downstream task), as reported in Table \ref{tab:main_table_results}. The findings clearly indicate that there is no significant decrease in performance when using shared weights, and in some cases, weight sharing even leads to improvements. This validates the claim that sharing the weights of the encoder across filters can effectively reduce computational load without compromising on performance.


% 


 It is important to highlight that the motivation for learning using multiple filters stems from models like \gprgnn, which aim to learn task-specific representations by effectively utilizing information from different parts of the eigenspectrum. In the case of \ourmethod, we demonstrate that it is possible to learn these representations in an unsupervised and task-agnostic manner. The only task-specific aspect lies in how these learned representations are combined, utilizing a weighted sum combination method (see \ref{subsec:supervised_representation_learning}) in the downstream supervised task.

==> sections/experiments.tex <==
\section{Experimental Results}
\label{sec:experimental_results}

\textbf{Training Details}: We define a single-layer graph convolutional network (\gcn) with shared weights ($\Theta$) across all filters in the filter bank ($\filter{}$) as our encoder. Therefore, the encoder can be expressed as follows: $\enc(\feat, \filter{i}) = \sigma(\filter{i}\feat\Theta)$. It is important to note that $\filter{i}$ represents a normalized filter with self-loops, which ensures that its eigenvalues are within the range of [0, 2]. The non-linearity function $\sigma$ refers to the parametric rectified linear unit (\prelu) \cite{misc:prelu}. As we work with a single graph, we obtain the positive samples by sampling nodes from the graph. Using these sampled nodes, we construct a new adjacency list that only includes the edges between these sampled nodes in filter $\filter{i}$. On the other hand, the corruption function $\mathcal{C}$ operates on the same sampled nodes. However, it randomly shuffles the node features instead of perturbing the adjacency list. Similar to \cite{gc:dgi}, we employ a straightforward readout function that involves averaging the representations across all nodes for a specific filter $\filter{i}$: $\mathcal{R}(\mathbf{H}_{i}) = \sigma\left(\frac{1}{N}\sum_{j=0}^{N}h_{j}^{\filter{i}}\right)$ where $\sigma$ denotes the sigmoid non-linearity. We utilize a bilinear scoring function, whose parameters are also shared across all filters:
\begin{equation}
    \label{eq:bilinear}
    D_{\omega}(h_{j}^{\filter{i}}, h_{g}^{\filter{i}}) = \sigma(h_{j}^{\filter{i}T}\mathbf{W}h_{g}^{\filter{i}})
\end{equation}

We learn the encoder and discriminator parameters by optimising Eq. \ref{eq:total_loss}. While we could use various filter banks, we specifically employ the filter bank corresponding to \gprgnn~($\filter{\gprgnn}$) for all our experiments. However, we also conduct an ablation study (see \ref{subsec:exp_filter_banks}) to compare the performance when using $\filter{\gprgnn}$ versus $\filter{\bernnet}$. For more detailed training information, please refer to the supplementary material.


%%%%%%%%%%%%%

We conducted a series of comprehensive experiments to evaluate the effectiveness and competitiveness of our proposed model compared to \sota~models and methods. These experiments address the following research questions: \textbf{[RQ1]} How does \ourmethod, perform compared to \sota~unsupervised models? \textbf{[RQ2]} Can we perform satisfactorily even with lower dimensional representations using projections such as RFF? \textbf{[RQ3]} Does shared encoder decrease performance? \textbf{[RQ4]} What is the computational efficiency gained by using lower dimensional representations compared to methods that rely on higher dimensional representations? \textbf{[RQ5]} Can alternative filter banks be employed to recover good quality representations?

%%%%%%%%%%%%%%%%%%

\textbf{Datasets and Setup:} We evaluated our model on a diverse set of real-world datasets, which include both heterophilic and homophilic networks, to assess its effectiveness. Similar to previous works, we utilized the node classification task as a proxy to evaluate the quality of the learned representations. Please refer to the supplementary material for detailed information about the benchmark datasets.


% The heterophilic datasets include \textbf{\texas}, \textbf{\cornell}, \textbf{\wisconsin}, \textbf{\chameleon}, \textbf{\squirrel}, \textbf{\romanempire} and \textbf{\minesweeper}. For \texas, \cornell, \wisconsin, \chameleon~and \squirrel~we use the 10 random splits (48\%, 32\%, 20\% of nodes for train/validation/test set) from \cite{d:geomgcn}. For \romanempire~and \minesweeper~we use the 10 random splits from \cite{d:criticalheterophily}. We also evaluate on 4 homophilic datasets: \textbf{\cora}, \textbf{\citeseer}, \textbf{\pubmed}, and Amazon Electronics – \textbf{\computers} borrowed from \cite{d:supergat}. To compare model performance, we report the mean and standard deviation of the test accuracy across the splits. Dataset statistics are provided in the appendix.

The heterophilic datasets used in our evaluation include \textbf{\chameleon}, \textbf{\squirrel}, \textbf{\romanempire}, and \textbf{\minesweeper}. For  \chameleon~and \squirrel, we adopted the ten random splits (with 48\%, 32\%, and 20\% of nodes allocated for the train, validation, and test sets, respectively) from \cite{d:geomgcn}. For \romanempire~and \minesweeper, we used the ten random splits provided in \cite{d:criticalheterophily}. Additionally, we evaluated our model on four homophilic datasets: \textbf{\cora}, \textbf{\citeseer}, and \textbf{\pubmed}, as borrowed from \cite{d:supergat}. We report the mean and standard deviation of the test accuracy across different splits. Please refer to the supplementary material for detailed statistics of each dataset.

%%%%%%

\textbf{Baselines:} In our comparison against baselines, we considered common unsupervised approaches, such as \deepwalk~and \nodevec, and state-of-the-art mutual information-based methods, namely \dgi, \mvgrl, \grace, and \sugrl. We also include the performance numbers of the widely used \gcn for reference. It is important to note that unless explicitly mentioned, we set the representation size to 512 dimensions for all reported results, consistent with previous work. Please refer to the supplementary material for detailed comparisons with other supervised methods and the link to our codebase. 

% In our study, we conducted a thorough comparison of our model against various baselines. We considered common unsupervised approaches, such as \deepwalk~and \nodevec, as well as state-of-the-art mutual information-based methods, namely \dgi, \mvgrl, \grace, and \sugrl. Additionally, for reference, we included the performance numbers of the widely used \gcn. Comparisons with other supervised methods can be found in the appendix. Please note that unless explicitly mentioned, all reported numbers come from setting the representation size to 512 dimensions, in line with previous work. \textbf{Please note that the link to our codebase can be found in the supplementary material}.



%%%%%%%
\subsection{RQ1: \ourmethod~versus \sota~Methods} 
\label{subsec:exp_sota}




%%%%%%%%%

\begin{table}[!ht]    
    \renewcommand*{\arraystretch}{1.2}
    \centering
    \caption{Contains node classification accuracy percentages on homophilic and heterophilic datasets. \ourmethod$_{32}$ and \ourmethod$_{128}$ refer to \ourmethod~trained with 32 and 128 dimensional representations, respectively, and then projected using RFF. The remaining models are trained at 512 dimensions. Higher numbers indicate better performance. It is worth noting that \ourmethod~achieves superior performance or remains competitive with the baseline methods in all cases. The rightmost column Av. $\Delta_{gain}$ represents the average accuracy $\%$ gain of \ourmethod~over the model in that row, averaged across the different datasets. \tblfirst{Blue}, \tblsecond{Red} and \tblthird{Green} represent the $1^{\text{st}}$, $2^{\text{nd}}$ and $3^{\text{rd}}$ best performing models, for a particular dataset.}
    \resizebox{\linewidth}{!}{    \begin{tabular}{cccccccc|c}
    \hline
        & \multicolumn{4}{|c|}{\textsc{Heterophilic Datasets}} & \multicolumn{3}{c|}{\textsc{Homophilic Datasets}} & \\
         & \multicolumn{1}{|c}{\squirrel} & \chameleon & \romanempire & \multicolumn{1}{c|}{\minesweeper} & \cora  & \citeseer & \pubmed & Av. $\Delta_{gain}$ \\ \hline
        \deepwalk & 38.66 (1.44) & 53.42 (1.73) & 13.08 (0.59) & 79.96 (0.08) & 83.64 (1.85) & 63.66 (3.36) & 80.85 (0.44) & 16.35\\ 
        \nodevec & 42.60 (1.15) & 54.23 (2.30) & 12.12 (0.30) & 80.00 (0.00) & 78.19 (1.14) & 57.45 (6.44) & 73.24 (0.59) & 18.56\\ 
        \dgi & 39.61 (1.81) & 59.28 (1.23) & 47.54 (0.76) & 82.51 (0.47) & 84.57 (1.22) & \tblthird{73.96 (1.61)} & 86.57 (0.52) & 7.67\\ 
        \mvgrl & 39.90 (1.39) & 54.61 (2.29) & \tblsecond{68.50 (0.38)} & \tblfirst{85.60 (0.35)} & \tblsecond{86.22 (1.30)} & \tblfirst{75.02 (1.72) }& \tblsecond{87.12 (0.35)} & 4.39\\ 
        \grace & \tblfirst{53.15 (1.10)} & \tblsecond{68.25 (1.77)} & 47.83 (0.53) & 80.22 (0.45) & 84.79  (1.51) & 67.60 (2.01) & \tblthird{87.04 (0.43)} & 5.54\\ 
        \sugrl & 43.13 (1.36) & 58.60 (2.04) & 39.40 (0.49) & 82.40 (0.58) & 81.21 (2.07) & 67.50 (1.62) & 86.90 (0.54) & 9.80\\ \hline
        \ourmethod$_{32}$ & \tblthird{48.89 (1.55)} & 65.66 (2.52) & 67.67 (0.77) & \tblthird{85.28 (0.71)}  & 82.56 (0.87) & 71.25 (2.20) & 84.18 (0.53) & 3.18\\ 
        \ourmethod$_{128}$ & 48.78 (2.48) & \tblthird{66.03 (2.19)} & \tblthird{68.10 (1.09)}& 85.16 (0.58) & \tblthird{86.14 (1.13)} & 73.34 (1.91)  & 85.41 (0.52)  & 2.11\\ 
        \ourmethod & \tblsecond{52.23} (1.19) & \tblfirst{68.55  (1.87)} & \tblfirst{70.99 (0.52)} & \tblsecond{85.58 (0.49)} & \tblfirst{87.00 (1.24)} & \tblsecond{74.77 (2.00)} & \tblfirst{88.60 (0.44)}& 0.00\\ \hline
    \end{tabular}}
    \label{tab:main_table_results}
\end{table}




%%%%%%%


\begin{table}[!ht]    
    \renewcommand*{\arraystretch}{1.2}
    \centering
    \caption{Comparison of Node classification accuracy percentages with the widely used supervised model \gcn. Despite not having access to task specific labels, \ourmethod~learns good quality representations.}
    \resizebox{\linewidth}{!}{    \begin{tabular}{cccccccc}
    \hline
         & \squirrel & \chameleon & \romanempire & \minesweeper & \cora  & \citeseer & \pubmed \\ \hline

        \gcn & 47.78 (2.13) & 61.43 (2.70) & \textbf{73.69 (0.74)} & \textbf{89.75 (0.52)} & \textbf{87.36 (0.91)} & \textbf{76.47 (1.34)} & 88.41 (0.46) \\ 
        \ourmethod & \textbf{52.23 (1.19)} & \textbf{68.55  (1.87)} & 70.99 (0.52) & 85.58 (0.49) & 87.00 (1.24) & 74.77 (2.00) & \textbf{88.60 (0.44)} \\ \hline
    \end{tabular}}
    \label{tab:gcn_table_results}
\end{table}



We analyzed the results in Table \ref{tab:main_table_results} and made important observations. Across homophilic and heterophilic datasets, \ourmethod~consistently outperforms several \sota~unsupervised models, except in a few cases where it achieves comparable performance. We want to emphasize the rightmost column of the table, which shows the average percentage gain in performance across all datasets. This metric compares the improvement that \ourmethod~provides over each baseline model for each dataset and averages these improvements. This metric highlights the performance consistency of \ourmethod~across diverse datasets. No other baseline model achieves the same consistent performance across all datasets as \ourmethod. Even the recent state-of-the-art contrastive models \grace~and \sugrl~experience average performance drops of approximately 5\% and 10\%, respectively. This result indicates that \ourmethod~learns representations that exhibit high generalization and task-agnostic capabilities. Another important observation is the effectiveness of RFF projections in improving lower dimensional representations. We compared \ourmethod~at different dimensions, including $\ourmethod_{32}$ and $\ourmethod_{128}$, corresponding to learning 32 and 128-dimensional embeddings, respectively, in addition to the baseline representation size of 512 dimensions. Remarkably, even at lower dimensions, \ourmethod~with RFF projections demonstrates competitive performance across datasets, surpassing the 512-dimensional baselines in several cases. This result highlights the effectiveness of RFF projections in enhancing the quality of lower dimensional representations. Section~\ref{subsec:exp_rff_projections} discusses more insights about the effectiveness of RFF projections. Furthermore, we include the widely used supervised model, \gcn, in Table \ref{tab:gcn_table_results} as a benchmark for comparison. Notably, \ourmethod~outperforms \gcn~on heterophilic datasets, except for \romanempire~and \minesweeper, while achieving competitive performance on homophilic datasets. Please refer to supplementary material for detailed comparisons with supervised methods.

\subsection{RQ2: RFF Projections on Lower Dimensional Representations}
\label{subsec:exp_rff_projections}
\begin{table}[!ht]
    \renewcommand*{\arraystretch}{1.2}
    \small
    \centering
    \caption{Node classification accuracy percentages with and without using Random Fourier Feature projections (on 32 dimensions). A higher number means better performance. 
 The performance is improved by using RFF in almost all cases, indicating the usefulness of this transformation}
    \begin{tabular}{cccccc}
    \hline
         & \textsc{rff} & \cora & \citeseer  & \squirrel & \chameleon \\ \hline
        \dgi & $\times$ & \textbf{81.65 (1.90)} & 65.62 (2.39) & 31.60 (2.19) & 45.48 (3.02) \\ 
        ~ & \checkmark & 81.49 (1.96) & \textbf{66.50 (2.44)} & \textbf{38.19 (1.52)} & \textbf{56.01 (2.66)} \\ \hline
        \mvgrl & $\times$ & \textbf{81.03 (1.29)} & 72.38 (1.68) & 37.20 (1.22) & 49.65 (2.08) \\ 
        ~ & \checkmark & 80.48 (1.71) & \textbf{72.54 (1.89)} & \textbf{39.53 (1.04)} & \textbf{56.73 (2.52)} \\ \hline
        \sugrl & $\times$ & 65.35 (2.41) & 42.84 (2.57) & 31.62 (1.47) & 43.20 (1.79) \\ 
        ~ & \checkmark & \textbf{70.06} (1.24) & \textbf{47.03} (3.02) & \textbf{38.50 (2.19)} & \textbf{51.01 (2.26)} \\ \hline
        \grace & $\times$ & 76.84 (1.09) & 58.40 (3.05) & 38.20 (1.38) & 53.25 (1.58) \\ 
        ~ & \checkmark & \textbf{79.15 (1.44)} & \textbf{63.66 (2.96)} & \textbf{51.56 (1.39)} & \textbf{67.39 (2.23)} \\ \hline
        \ourmethod & $\times$ & \textbf{82.88  (1.42)} & 70.32 (1.98) & 39.38 (1.35) & 53.27 (2.40) \\ 
        ~ & \checkmark & 82.56 (0.87) & \textbf{71.25 (2.20)} & \textbf{48.89 (1.55)} & \textbf{65.66 (2.52)} \\ \hline
    \end{tabular}
\label{tab:rff_table_32}    
\end{table}



In this section, we analyse the performance of unsupervised baselines using 32-dimensional embeddings with and without RFF projections (see Table \ref{tab:rff_table_32}). Despite extensive hyperparameter tuning, we could not replicate the results reported by \sugrl, so we present the best results we obtained. Two noteworthy observations emerge from these tables. Firstly, it is evident that lower dimensional embeddings can yield meaningful and linearly separable representations when combined with simple RFF projections. Utilising RFF projections enhances performance in almost all cases, highlighting the value captured by \mi-based methods even with lower-dimensional embeddings. Secondly, \ourmethod~consistently achieves superior or comparable performance to the baselines, even in lower dimensions. Notably, this includes \sugrl, purported to excel in such settings. However, there is a 2-3\% performance gap between \grace~and our method for the \squirrel~and \chameleon~datasets. While \grace~handles heterophily well at lower dimensions, its performance deteriorates with homophilic graphs, unlike \ourmethod~which captures lower frequency information effectively. Additionally, our method exhibits computational efficiency advantages for specific datasets in lower dimensions. Please refer to the supplementary material for more details. Overall, these findings highlight the potential of RFF projections in extracting useful information from lower dimensional embeddings and reaffirm the competitiveness of \ourmethod~over the baselines.


\subsection{RQ3: Sharing Weights Across Filter Specific Encoders}
\label{subsec:enc_weight_sharing}
\begin{table}[ht]
    \small
    \renewcommand*{\arraystretch}{1.2}
    \centering
    \caption{A comparison of the performance on the downstream node classification task using independently trained encoders and weight sharing across encoders is shown. The reported metric is accuracy. In both cases, the embeddings are combined using the method described in \ref{subsec:supervised_representation_learning}}
    \begin{tabular}{ccccc}
    \hline
         & \cora & \citeseer & \squirrel & \chameleon \\ \hline
        \textsc{Independent} & 86.92 (1.10) $\%$ & 75.03 (1.75) $\%$ & 50.52 (1.51) $\%$ & 66.86 (1.85) $\%$ \\ 
        \textsc{Shared} & 87.00 (1.24) $\%$ & 74.77 (2.00) $\%$ & 52.23 (1.19) $\%$ & 68.55 (1.87) $\%$ \\ \hline
    \end{tabular}
\label{tab:independent_vs_shared}
\end{table}
Our method proposes to reduce the computational load by sharing the encoder weights across all filters. It stands to reason whether sharing these weights causes any degradation in performance. We present the results with shared and independent encoders across the filters in Table \ref{tab:independent_vs_shared} to verify this. The findings indicate no significant decrease in performance when using shared weights, and in some cases, it even leads to improvements, validating the use of shared encoders.

% To validate the claim that it is possible to reduce the computational load by sharing the weights of the encoder across filters, without drop in performance, the experiment in Table \ref{tab:independent_vs_shared} was performed. Independent encoders were trained on each filter separately, and the embeddings were combined using the alpha combination \todo as described previously. The performance is then compared with the shared encoder results, which were also reported in Table \ref{tab:main_table_heterophilic} and Table \ref{tab:main_table_homophilic}. It is clear that there is no noticeable drop of performance, and in some cases the weight sharing leads to improvements.

\subsection{RQ4: Computational 
Efficiency} 
\label{subsec:exp_computational_efficiency}

\begin{table}[!ht]
    \small
    \renewcommand*{\arraystretch}{1.2}
    \centering
    \caption{Mean epoch time (in milliseconds) averaged across 20 trials with different hyperparameters. A lower number means the method is faster. Even though our method is slower at 512 dimensions, using 128 and 32 dimensional embeddings significantly reduces the mean epoch time. Using RFF as described in \ref{subsec:exp_rff_projections} we are able to prevent the performance drops experienced by \dgi~and \mvgrl.}
    \begin{tabular}{ccccccc}
    \hline
          & DGI & MVGRL & \ourmethod & \ourmethod$_{128}$ & \ourmethod$_{32}$ \\ \hline
        \cora & 38.53 (0.77) & 75.29 (0.56) & 114.38 (0.51) & 20.10 (0.46) & 11.54 (0.34) \\ 
        \citeseer & 52.98 (1.15) & 102.41 (0.99) & 156.24 (0.56) & 30.30 (0.60) & 17.16 (0.51) \\ 
        \squirrel & 87.06 (2.07) & 168.24 (2.08) & 257.65 (0.76) & 47.72 (1.40) & 23.52 (1.14) \\ 
        \chameleon & 33.08 (0.49) & 64.71 (1.05) & 98.36 (0.64) & 18.56 (0.39) & 11.63 (0.48) \\ \hline

    \end{tabular}
\label{tab:computational_efficiency}
\end{table}

% To assess the computational efficiency of the different methods, we analyzed the computation time, as summarized in table Table \ref{tab:computational_efficiency}. The key metric of interest in this analysis is the mean epoch time. We compare our method with other mutual information based methods like \dgi~and \mvgrl. As mentioned earlier, there is an expected increase in computation time, from \dgi~to \mvgrl~to \ourmethod, corresponding to the increase in the number of augmentation views that are accessible to the model. However, as shown previously, using RFF we are able to obtain competitive performance even at lower dimensions. Therefore, comparisons with our method at 128 and 32 dimensions are also included in this table. It is easily noticeable that our method at both 128 and 32 dimensions is faster than both \dgi and \mvgrl, which are restricted to higher dimensional representations to achieve good performance. Thus, in summary, \ourmethod is computationally efficient as a result of working with lower dimensional representations. Further comparisons to other unsupervised models like \grace and \sugrl are present in the appendix.

To assess the computational efficiency of the different methods, we analyzed the computation time and summarized the results in Table \ref{tab:computational_efficiency}. The key metric used in this analysis is the mean epoch time: the average time taken to complete one epoch of training. We compared our method with other \mi~based methods such as \dgi~and \mvgrl. Due to the increase in the number of augmentation views, there is an expected increase in computation time from \dgi~to \mvgrl~to \ourmethod. However, as demonstrated in \ref{subsec:exp_rff_projections}, using RFF projections allows us to achieve competitive performance even at lower dimensions. Therefore, we also included comparisons with our method at 128 and 32 dimensions in the table. It is evident from the results that our method, both at 128 and 32 dimensions, exhibits faster computation times compared to both \dgi~and \mvgrl, which rely on higher-dimensional representations to achieve good performance. This result indicates that \ourmethod~is computationally efficient due to its ability to work with lower-dimensional representations. During training, our method, $\ourmethod_{32}$, is $\sim3$x faster than \dgi~and $\sim{6}$x times faster than \mvgrl. Despite the faster computation, $\ourmethod_{32}$ also exhibits an average performance improvement of around $2\%$ across the datasets over all methods considered in our experiments. Please refer to the supplementary material for additional comparisons to other unsupervised models.



\subsection{RQ5: Experiments on Other Filter Banks}
\label{subsec:exp_filter_banks}

\begin{table}[!ht]
    \small
    \renewcommand*{\arraystretch}{1.2}
    \centering
    \caption{Accuracy percentage results using other filter banks for \ourmethod. $\filter{\bernnet}^3$ refers to the $\filter{\bernnet}$ filter bank (Section~\ref{subsec:filter_banks}) with $K$ set to $3$ and $\filter{\bernnet}^{11}$ refers to $K$ set to $11$.}
    \begin{tabular}{ccccc}
    \hline
         & \cora  & \citeseer & \squirrel & \chameleon \\ \hline
        $\filter{\bernnet}^3$ & 85.13 (1.26) & 73.38 (1.81) & 37.07 (1.29) & 53.95 (2.78) \\ 
        $\filter{\bernnet}^{11}$ & 86.62 (1.59) & 73.97 (1.43) & 43.48 (3.80) & 62.13 (3.66) \\ 
        $\filter{\gprgnn}$ & 87.00 (1.24) & 74.77 (2.00) & 52.23 (1.19) & 68.55  (1.87) \\ \hline
    \end{tabular}
\label{tab:other_filter_banks}    
\end{table}

% To demonstrate \ourmethod~ being a general framework, flexible to the kind and quantity of filters, we conducted an experiment using Bernstein filters, in Table \ref{tab:other_filter_banks}. We find that that using $\filter{\gprgnn}$ shows improvements over using Bernstein filters, but it is nonetheless competitive with previous unsupervised baselines. We also find that the quantity of filters plays a role, as 11 bernstein filters capture more of the eigenspectrum than 3.

To showcase the versatility of our proposed framework, we conducted an experiment using Bernstein filters, as detailed in Table \ref{tab:other_filter_banks}. The results indicate that using $\filter{\gprgnn}$ leads to better performance than Bernstein filters. We believe that the reason this is happening is due to the latent characteristics of the dataset. \cite{gf:bernnet,gf:ppgnn} have shown that datasets like \chameleon~and \squirrel~need frequency response functions that give more prominence to the tail-end spectrum. $\filter{\gprgnn}$ are more amenable to these needs, as demonstrated in \cite{gf:ppgnn}. However, datasets requiring frequency response similar to comb filters may be better approximated by $\filter{\bernnet}$ as their basis gives uniform prominence on the entire spectrum. Please refer to the supplementary material, which shows the basis frequency responses of these two filter banks, with more clarification. Therefore, although $\filter{\gprgnn}$ gives better performance for these datasets, there could be datasets where $\filter{\bernnet}$ could do better. Hence, we proposed a general framework that can work with any filter bank.

% To showcase the versatility of our proposed framework, we conducted an experiment using Bernstein filters, as detailed in Table \ref{tab:other_filter_banks}. The results indicate that using $\filter{\gprgnn}$ leads to better performance compared to Bernstein filters. We believe that the reason this is happening lies in the kind of polynomials that can be learnt by these filter banks. While theoretically, these filter banks should be able to a approximate any polynomial frequency response function within a certain desired degree, due to the nature of the bases and the intricacies of gradient descent optimization, we believe that certain response functions are easier to approximate than others, leading to local minima problems if the desired function is too complex to learn. As shown in \cite{gf:bernnet}, the learnt filter response function required by datasets like squirrel, chameleon, cora and citeseer is more dumbell shaped, giving importance to the tail-ends of the spectrum. The bases filters associated with \gprgnn~are more in line with this requirement, since they focus on the tail ends of the spectrum. In contrast the \bernnet filters also give importance to the middle of the spectrum. Thus using the Bernstein bases to approximate the required filters may be a more difficult learning task than using the \gprgnn~filters. The focus on the middle part of the spectrum is less pronounced as the number of Bernstein bases increases, in line with the observation that as you increase the number of Bernstein bases, the accuracy on the downstream task increases. For further reading, we refer the reader to \cite{gf:ppgnn}.




==> sections/method.tex <==
\section{Simple Filter-Based Augmentations for Unsuprvised Node Representation Learning}


\subsection{Filter learning on Graphs}

Let $\nadj = \eigenU\adjS\eigenU^T$ be the eigendecomposition of $\nadj$, and $\adjS = diag([\lambda_1, \lambda_2, ..., \lambda_n])$. Let $\nlap$ be the symmetric normalised Laplacian, $\nlap=\eye-\nadj$. The spectral convolution of $\feat$ on the adjacency matrix $\adj$ can be defined via a filter function $g: \mathbb{R}^{n \times n} \rightarrow \mathbb{R}^{n \times n}$, which operates on the eigenvalues in the spectral domain \cite{gf:gsp_shuman, gf:gsp_tremblay}, and the reference operater $\nadj$ as:

\begin{equation}
    \label{eq:gen_filter}
    Z =  \eigenU g(\adjS) \eigenU^T \feat
\end{equation}

However, performing the eigendecomposition for large graphs is computationally infeasible. Instead, the filter function can be modified such that $g: \mathbb{R} \rightarrow \mathbb{R}$, and $g$ is a polynomial function of order $K$. Then the convolutional operator is defined as follows: 

\begin{equation}
    \label{eq:pol_filter}
    Z =  \eigenU g(\adjS) \eigenU^T = \eigenU diag([g(\lambda_1), g(\lambda_2), ..., g(\lambda_n)] = \sum_{i=0}^{k}\alpha_{i}(\nadj)^{i}\feat
\end{equation}

Note that, $\alpha_i$'s are learnable coefficients of the polynomial filter function $g : g(\lambda) = \sum_{i=0}^{k}\alpha_{i}\lambda^{i}$. Additionally, note that the polynomial filters span the entire eigenspectrum, thereby having the ability to aggregate information from different parts of the eigenspectrum \addfig~(Standard basis, Bernstein basis ). Basis the downstream task, the filter function can learn to accentuate or attenuate, certain frequencies (eigenvalues) in order to obtain richer representations, which in turn leads to obtaining performance improvements for the task at hand. This follows from the work proposed in \cite{gf:gprgnn, gf:ppgnn, gf:bernnet}. While, polynomial filters can learn any other polynomial filters, a few problems \cite{gf:bernnet} in learning a free form solution are a) there are no explicit constraints on the form of the polynomial, thereby leading to poor controlability, b) the learnt filters are not interpretable and c) the filters learnt can be ill posed. 

A solution to the above problems as proposed by \cite{gf:bernnet} is to learn a a weighted combination of a bank of polynomial filters, where each filter is itself a well posed filter function. Let the $i$'th filter in the filter bank be defined as $\filter{i}$. Note that $\rho(\filter{i}) \leq 2$, where $\rho(.)$ is the spectral radius and that the smallest eigenvalue of $\filter{i}$ is greater than $0$. The convolutional operator on the bank of $K$ polynomial filters is defined as follows:

\begin{equation}
    \label{eq:pol_filter_bank}
    Z =   \sum_{i=0}^{K}\alpha_{i}\filter{i}\feat
\end{equation}

\bernnet~\cite{gf:bernnet} is a specific instantiation of a bank of polynomial filters (of order $K$) which has the following convolutional operator: 

\begin{equation}
    \label{eq:bernnet}
    Z =   \sum_{i=0}^{K}\alpha_{i}\frac{1}{2^{K}}\binom{K}{i}(2\eye-\nlap)^{k-i}(\nlap)^{i}\feat
\end{equation}

Note that $\alpha_i$'s are learnable positive coefficients.



%%% ENCODERS %%%%



\subsection{Encoders}

Our method builds upon \cite{vc:infomax, gc:dgi}, where we maximize the mutual information patch level representations (node representations obtained from the encoder) and the global filter representations, for each filter in the filter bank $\filter{} = [\filter{1}, \filter{2}, ... \filter{K}]$. 

We learn an encoder per filter such that the mutual information between the input data and the output of the encoder is maximised. Hence, for the $i$'th filter we learn an encoder, $\enc: \mathcal{X}_i \rightarrow \mathcal{X}_{i}'$ where $\theta$ represents the learnable parameters of the encoder. Note that $\mathcal{X}_{i}$ denotes the set of examples provided, where $\mathcal{X}_{i}: \{\sampjointfilt{ij} \in \mathcal{X}_{i}, \forall j\}$, with empirical probability distribution $\mathbb{P}_{i}$. This implies that $\mathcal{X}_{i}$ contains sets of filters (and their corresponding nodes and node features), drawn from a joint distribution of features and node representations corresponding to $[\feat, \filter{i}]$. $\mathcal{X}_i$ defines the set of representations learnt by the encoder on utilising feature information as well as topological information from the samples, sampled from the joint distribution $\mathbb{P}_{i}$. Following \cite{misc:infomax_principle, vc:infomax, gc:dgi}, the goal is to find $\theta$, such that the mutual information between $\featfilter{i}$ and $\encproj{i}$, represented as $\mathcal{I}_{i}(\featfilter{i}, \encproj{i})$ is maximised. Note that the set of nodes (and their corresponding features) are shared across all features. Due to unavailability of the distribution of the data as well as the learned representations, computing the exact value of mutual information is not feasible. As shown in \addcite (Nowozin and Donsaker Vardhan) it is possible to estimate \mi~ via Jenson-Shannon MI estimator, defined as follows:

\begin{equation}
    \label{eq:mi_jsd}
    \begin{split}
        \mathcal{I}^{JSD}_{i, \theta, \omega}(\featfilter{i}, \encproj{i}):= \mathbb{E}_{\mathbb{P}_{i}}[-\text{sp}(T_{\theta, \omega}(\sampjointfilt{ij}, \encsamp{ij}]- \\ \mathbb{E}_{\mathbb{P}_{i} \times \mathbb{\tilde{P}}_{i}}[\text{sp}(T_{\theta, \omega}(\sampjointcorr{ij},  \encsamp{ij})]
        \end{split}
\end{equation}

Where, $T: \mathcal{X}_{i} \times \mathcal{X'}_{i} \rightarrow \mathbb{R}$ is a discriminator function with, with learnable parameters $\omega$. Note that $[\tilde{\feat_{ij}}, \tilde{\filter{ij}}]$ is an input sampled from $\mathbb{\tilde{P}}_{i}$, which is a marginal of the joint distribution of both the input data and the learned node representations, and that sp(.) denotes the softplus function \addcite. Also note that $T_{\theta, \omega} = D_{w} \circ (\mathcal{R}(\encsamp{ij}), \encsamp{ij})$, where $\mathcal{R}$ denotes the readout function which summarizes all the patch level (node level) representations by aggregating and distilling the information into a global (graph level) representation.

Concretely, for each filter, we obtain patch level representations by passing the filter specific topology as well as the associated node features to the encoder, $\mathbf{H}_{i} = \enc(\feat_{i}, \filter{i}) = \{h^{\filter{i}}_{1}, h^{\filter{i}}_{2}, ..., h^{\filter{i}}_{n}\}$. To obtain the global representations, we utilize a readout function $\mathcal{R}: \mathbb{R}^{N \times d'} \rightarrow \mathbb{R}^{d'}$, which combines and distills information into a global representation $h_{g}^{F_i} = \mathcal{R}(\mathbf{H}_{i}) = \mathcal{R}(\encproj{i})$. As a substitute for maximising the mutual information between the local and global representation, we utilize a learnable discriminator, $D_{\omega}: \mathbb{R}^{d'} \times \mathbb{R}^{d'} \rightarrow \mathbb{R}$, where $D_{\omega}(., .)$ denotes the joint probability score of the global representation and the node specific patch representation. This joint should be optimised to be higher for global representations and local representations obtained from the same filter as opposed to the joint of the global representations obtained from a filter and local representation obtained from any other arbitrary filter.

While our approach would generate representations that capture the entire eigenspectrum, storing separate patch level representations (per filter) can become prohibitively expensive for large graphs. Moreover, generally, contrastive learning methods require higher dimensions, increasing both the computational cost of training as well as storage. To tackle the first issue, we share the parameters $\theta, \omega$ of the encoder and the discriminator respectively across all filters. This is inspired by works such as \cite{gf:gprgnn, gf:bernnet} where the encoder is shared across multiple filters. We believe that $\theta$ can be shared across all the encoders as each filter $\filter{i}$ projects the representations into its own corresponding Hilbert space in $\mathbb{R}^{d'}$. This allows us to reconstruct filter-specific representations as needed, while also reducing the computational and storage load. To combat the second problem, we first train our models to generate very low dimensional embeddings. Inspired by kernel methods, we use \rff~projections to lift these low dimensional embeddings to higher dimensions. \addref 

Negative samples for contrastive learning are obtained via a corruption function $\mathcal{C}: \mathbb{R}^{N \times d} \times \mathbb{R}^{N \times N}  \rightarrow \mathbb{R}^{M \times d} \times \mathbb{R}^{M \times M}$, such that $\sampjointcorr{ij}=\mathcal{C}(\feat, \filter{i})$. The corruption function is designed in such a way that the data generated from the corruption function is decorrelated from the input data. Hence to learn representations across all filters in the filter bank, we maximize the average of the estimate of \mi~across all filters (considering $K$ filters):

\begin{equation}
    \mathcal{I}_{\filter{}} = \frac{1}{K}\sum_{i=1}^{K} \mathcal{I}^{JSD}_{i, \theta, \omega}(\featfilter{i}, \encproj{i})
\end{equation}



\subsection{Projections into Higher Dimensional Spaces}

\paragraph{Kernel trick and Cover's theorem:} The kernel trick is a method that generates features for downstream algorithms that depend on only the inner product between all pairs of input points. It does this by utilising a positive definite function $k(\mathbf{x}, \mathbf{y})$ (where $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$) and a lifting function $\phi(.)$ so that the inner product between the lifted datapoints can be easily computed as follows: $\langle \phi(\mathbf{x}), \phi(\mathbf{y}) \rangle =  k(\mathbf{x}, \mathbf{y})$. By Cover's theorem \addcite~and Mercers theorem \addcite, there exists a non-linear map  $\phi(.)$, that lifts the input datapoints to a higher dimensional space where the transformed datapoints are linearly separable.  

As discussed in \addref~(Intro, prior section etc), for computational and storage efficiency we need to train our model to learn very low dimensional embeddings that contain information that would be utilised for downstream tasks. As discussed in \cite{misc:analysisrff}, there exist latent classes where each data point belongs to. These latent classes are defined to be a superset of set of classes defined for each downstream task. We believe that even for the current graph setting, these latent classes exist, and this notion of latent classes is also present in lower dimensional embeddings. However, while these lower dimensional embeddings contain this latent class information, this information is no longer linearly separable. Hence, to achieve good downstream performance, we need to project these embeddings to a higher dimensional space (where these latent classes would be linearly separable). We experimentally show this in section \addref~(Experiments).

In this entire ordeal the lifting function $\phi(.)$ becomes an important component, which should only add a minor computational load to the entire algorithm. Hence, we rely on \rff~projections \cite{misc:rff}, which approximate the map associated with the RBF kernel. Because of their design, they are very cheap and easy to compute adding to very little computational load. Random Fourier Features are defined as follows:

\begin{equation}
    \label{eq:rff}
    \phi(\mathbf{x}) = \text{cos}(\mathbf{w}^Tx + \tau)
\end{equation}

where $\mathbf{w} \sim N(0, \gamma^{2}\eye_d)$ and $\tau \sim \text{Unif}(0, 2\pi)$


%%% TRAINING %%%%

\subsection{Training Details}

We define the encoder to be a single layer \gnn~whose weights ($\Theta)$ are shared across each filter in the filter bank. Hence, the encoder is defined as follows:

\begin{equation}
    \label{eq:encoder}
    \enc(\feat, \filter{i}) = \sigma(\filter{i}\feat\Theta)
\end{equation}

Note that, $\filter{i}$ denotes a normalised filter with self loops such that the eigenvalues of the $\filter{i}$ are constrained between $[0, 2]$. The nonlinearity $\sigma$, denotes the \prelu~function \addcite. Since we work in a single graph setting, to obtain positive samples, we sample nodes from given graph. Basis the sampled nodes, we create a new adjacency list corresponding to the edges present between only these sampled nodes, in filter $\filter{i}$. The corruption function $\mathcal{C}$ operates on the same sampled nodes, however, the corruption function does not perturb the adjacency list, but randomly shuffles the nodes, thereby changing the topological structure of the graph. 

Similar to \cite{gc:dgi}, we utilize a simple readout function, where we average the representations cross all nodes, for a particular filter $\filter{i}$ :

\begin{equation}
    \label{eq:readout}
    \mathcal{R}(\mathbf{H}_{i}) = \sigma(\frac{1}{N}\sum_{j=0}^{N}h_{j}^{\filter{i}})
\end{equation}

where, $\sigma$ denotes the sigmoid \addcite~non-linearity. Following \addcite (Oord et. al.), we utilize a bilinear scoring function, whose parameters are also shared across all filters:

\begin{equation}
    \label{eq:bilinear}
    D_{\omega}(h_{j}^{\filter{i}}, h_{g}^{\filter{i}}) = \sigma(h_{j}^{\filter{i}}^{T}\mathbf{W}h_{g}^{\filter{i}})
\end{equation}

Following the work of \cite{gc:dgi, vc:infomax}, we use the following noise-contrastive objective, with a binary cross entropy loss, between positive samples (sampled from the joint) and the negative samples (product of marginals):

\begin{equation}
    \label{eq:loss}
    \mathcal{L} = \frac{1}{K} \left[\sum_{i=1}^{K} \frac{1}{N + M}\left( \sum_{j=1}^{N}\mathbb{E}_{(\feat, \filter{i})}[\text{log}(D_{\omega}(h_{j}^{\filter{i}}, h_{g}^{\filter{i}}))] + \sum_{j=1}^{M}\mathbb{E}_{(\tilde{\feat}, \tilde{\filter{i})}}[\text{log}(D_{\omega}(\tilde{h}_{j}^{\filter{i}}, h_{g}^{\filter{i}}))] \right) \right]
\end{equation}



\subsection{Combining Representations for Downstream Tasks}

Once the representations per filter are learnt, due to the shared weights of the encoder across each filter, we only need to store the encoder weights. Since we need to learn a filter function that can learn to modulate different parts of the eigenspectrum for the task at hand, we rely on learning schemes proposed in \cite{gf:gprgnn, gf:bernnet, gf:ppgnn}, where a weighted combination of filter specific representation is learnt. Hence, the combined representations we learn for the downstream task are as follows (for $K$ filters):

\begin{equation}
    Z = \sum_{i=1}^{K}\alpha_{i}\phi(\sigma(\filter{i}X\Theta) + \alpha_{0} \phi(X\Theta)
\end{equation}

Note that $\alpha_{i}$'s are learnable parameters. Also note that $\phi(.)$ represents the \rff~projection or an identity transformation based on whether $\filter{i}X\Theta$ is low dimensional or not. These embeddings are then passed to a logistic regression model, where both $\alpha_{i}$'s and the weights of the logistic regression model are tuned. Note that, one could also perform an \rff~projection after combining all the embeddings, and we show such an abalation study in \addref. For additional details please refer to the appendix. 

\addalg





\subsection{Preliminaries}
\begin{itemize}
    \item Define problem setting
    \item Define filters, filter banks, emphasize that filter weights are a requirement of downstream tasks. 
\end{itemize}

\subsection{Contrastive Learning Framework}
\begin{itemize}
    \item Define encoders, talk about patches, push forward measure, for each augmentation (i.e), each filter.
    \item Training: Define loss function, and define negative sampling. 
    \item Talk about why RFF, (have multiple filter augmentations, computational load). Experimentally find that its not linearly seperable in the lower dimension. Cover's theorem, RFF expression
    \item Top it off with Algorithm (add a conditional statement for RFF (depending on dimension size)
\end{itemize}


==> sections/proposed_approach.tex <==
\section{Proposed Approach}

The following section delineates the process of unsupervised representation learning. Post that, we give details on how the representations learned from each filter bank is used in downstream tasks using random feature maps.

\subsection{Unsupervised Representation Learning}

% Our method builds upon \cite{vc:infomax, gc:dgi}, where we maximize the mutual information patch level representations (node representations obtained from the encoder) and the global filter representations, for each filter in the filter bank $\filter{} = \{\filter{1}, \filter{2}, ... \filter{K}\}$. 

% In our approach, we extend the ideas presented in \cite{vc:infomax, gc:dgi}, which involve the maximization of mutual information between patch-level representations (encoder-based node representations) and global filter representations for each filter in the filter bank $\filter{} = \{\filter{1}, \filter{2}, ... \filter{K}\}$

% We learn an encoder per filter such that the mutual information between the input data and the output of the encoder is maximised. Hence, for the $i$'th filter we learn an encoder, $\enc: \mathcal{X}_i \rightarrow \mathcal{X}_{i}'$ where $\theta$ represents the learnable parameters of the encoder. Note that $\mathcal{X}_{i}$ denotes the set of examples provided, where $\mathcal{X}_{i}: \{\sampjointfilt{ij} \in \mathcal{X}_{i}, \forall j\}$, with empirical probability distribution $\mathbb{P}_{i}$. This implies that $\mathcal{X}_{i}$ contains sets of filters (and their corresponding nodes and node features), drawn from a joint distribution of features and node representations corresponding to $[\feat, \filter{i}]$. $\mathcal{X}_i$ defines the set of representations learnt by the encoder on utilising feature information as well as topological information from the samples, sampled from the joint distribution $\mathbb{P}_{i}$. Following \cite{misc:infomax_principle, vc:infomax, gc:dgi}, the goal is to find $\theta$, such that the mutual information between $\featfilter{i}$ and $\encproj{i}$, represented as $\mathcal{I}_{i}(\featfilter{i}, \encproj{i})$ is maximised. It is important to note that the set of nodes (and their corresponding features) are shared across all features. Since the exact distribution of the data and the learned representations are not available, it is not feasible to compute the exact value of the mutual information (\mi). However, as demonstrated in \cite{misc:donsaker_varadhan, misc:fgan}, it is possible to estimate the \mi~using the Jensen-Shannon MI estimator, defined as follows:


% \begin{equation}
%     \label{eq:mi_jsd}
%     \begin{split}
%         \mathcal{I}^{\textrm{JSD}}_{i, \theta, \omega}(\featfilter{i}, \encproj{i}):= \mathbb{E}_{\mathbb{P}_{i}}[-\text{sp}(T_{\theta, \omega}(\sampjointfilt{ij}, \encsamp{ij}]- \\ \mathbb{E}_{\mathbb{P}_{i} \times \mathbb{\tilde{P}}_{i}}[\text{sp}(T_{\theta, \omega}(\sampjointcorr{ij},  \encsamp{ij})]
%         \end{split}
% \end{equation}

% Here, $\mathcal{X}_{i}$ is the set of examples, each $\sampjointfilt{ij} \in \mathcal{X}_{i}$, following an empirical probability distribution $\mathbb{P}_{i}$. This set comprises filters and corresponding nodes and node features, drawn from a joint distribution of features and node representations $[\feat, \filter{i}]$

Our method \ourmethod~(\textbf{Fi}lter-based \textbf{G}raph \textbf{U}nsupervised \textbf{Re}presentation Learning)  builds on concepts introduced in \cite{vc:infomax, gc:dgi}, extending the maximization of mutual information between node and global filter representations for each filter in the filter bank $\filter{} = \{\filter{1}, \filter{2}, ... \filter{K}\}$. We construct an encoder for each filter to maximize the mutual information between the input data and encoder output. For the $i^{\textrm{th}}$ filter, we learn an encoder, $\enc: \mathcal{X}_i \rightarrow \mathcal{X}_{i}'$, denoted by learnable parameters $\theta$. In this context, $\mathcal{X}_{i}$ represents a set of examples, where each example $\sampjointfilt{ij} \in \mathcal{X}_{i}$ consists of a filter $\filter{i}$, its corresponding nodes and node features drawn from an empirical probability distribution $\mathbb{P}_{i}$, which captures the joint distribution of features and node representations $[\feat, \filter{i}]$. $\mathcal{X}_i$ defines the set of representations learnt by the encoder on utilizing feature information as well as topological information from the samples, sampled from the joint distribution $\mathbb{P}_{i}$. The goal, aligned with \cite{misc:infomax_principle, vc:infomax, gc:dgi}, is to identify $\theta$ that maximizes mutual information between $\featfilter{i}$ and $\encproj{i}$, or $\mathcal{I}_{i}(\featfilter{i}, \encproj{i})$. While exact mutual information (\mi) computation is unfeasible due to unavailable exact data and learned representations distributions, we can estimate the \mi~using the Jensen-Shannon MI estimator \cite{misc:donsaker_varadhan, misc:fgan}, defined as:

\begin{equation}
    \label{eq:mi_jsd}
    \begin{split}
        \mathcal{I}^{\textrm{JSD}}_{i, \theta, \omega}(\featfilter{i}, \encproj{i}):= \mathbb{E}_{\mathbb{P}_{i}}[-\text{sp}(T_{\theta, \omega}(\sampjointfilt{ij}, \encsamp{ij})]- \\ \mathbb{E}_{\mathbb{P}_{i} \times \mathbb{\tilde{P}}_{i}}[\text{sp}(T_{\theta, \omega}(\sampjointcorr{ij},  \encsamp{ij})]
        \end{split}
\end{equation}


Here, $T_{\omega}: \mathcal{X}_{i} \times \mathcal{X'}_{i} \rightarrow \mathbb{R}$ represents a discriminator function with learnable parameters $\omega$. Note that $[\tilde{\feat_{ij}}, \tilde{\filter{ij}}]$ is an input sampled from $\mathbb{\tilde{P}}_{i}$, which is a marginal of the joint distribution of the input data and the learned node representations. The function sp(.) corresponds to the softplus function~\cite{misc:softplus}. Additionally, $T_{\theta, \omega} = D_{w} \circ (\mathcal{R}(\encsamp{ij}), \encsamp{ij})$, where $\mathcal{R}$ denotes the readout function responsible for summarizing all node representations by aggregating and distilling information into a global filter representation.

\begin{wrapfigure}{r}{0.6\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/unsupervised_learning.pdf}
  \caption{Unsupervised learning of node embeddings by maximizing mutual information between node and graph representations over the graphs from the filter bank. Note that the parameter $\Theta$ is shared across all the filters.}\label{fig:unsupervised}
    \label{fig:unsup_learning}
\end{wrapfigure}

% Concretely, for each filter, we obtain patch level representations by passing the filter specific topology as well as the associated node features to the encoder, $\mathbf{H}_{i} = \enc(\feat_{i}, \filter{i}) = \{h^{\filter{i}}_{1}, h^{\filter{i}}_{2}, ..., h^{\filter{i}}_{n}\}$. To obtain the global representations, we utilize a readout function $\mathcal{R}: \mathbb{R}^{N \times d'} \rightarrow \mathbb{R}^{d'}$, which combines and distills information into a global representation $h_{g}^{F_i} = \mathcal{R}(\mathbf{H}_{i}) = \mathcal{R}(\encproj{i})$. As a substitute for maximising the mutual information between the local and global representation, we utilize a learnable discriminator, $D_{\omega}: \mathbb{R}^{d'} \times \mathbb{R}^{d'} \rightarrow \mathbb{R}$, where $D_{\omega}(., .)$ denotes the joint probability score of the global representation and the node specific patch representation. This joint should be optimised to be higher for global representations and local representations obtained from the same filter as opposed to the joint of the global representations obtained from a filter and local representation obtained from any other arbitrary filter.


In our approach, we first obtain node representations by feeding the filter-specific topology and associated node features into the encoder: $\mathbf{H}_{i} = \enc(\feat_{i}, \filter{i}) = \{h^{\filter{i}}_{1}, h^{\filter{i}}_{2}, ..., h^{\filter{i}}_{n}\}$. To obtain global representations, we employ a readout function $\mathcal{R}: \mathbb{R}^{N \times d'} \rightarrow \mathbb{R}^{d'}$, which combines and distills information into a global representation $h_{g}^{F_i} = \mathcal{R}(\mathbf{H}_{i}) = \mathcal{R}(\encproj{i})$. Instead of directly maximizing the mutual information between the local and global representations, we introduce a learnable discriminator $D_{\omega}: \mathbb{R}^{d'} \times \mathbb{R}^{d'} \rightarrow \mathbb{R}$, where $D_{\omega}(., .)$ represents the joint probability score between the global representation and the node-specific patch representation. This joint probability score should be higher when considering global and local representations obtained from the same filter, as opposed to the joint probability score between the global representation from one filter and the local representation from an arbitrary filter.

% \begin{figure}[]
%   \begin{minipage}{0.45\textwidth}
%     \raggedright
%     \includegraphics[width=1.1\linewidth]{figs/unsupervised_learning.pdf}
%     \caption{Unsupervised Learning of Node Embeddings}\label{fig:unsupervised}
%     \label{fig:figure1}
%   \end{minipage}%
%   \begin{minipage}{0.1\textwidth}
%     \centering
%      \includegraphics[width=1.2\linewidth]{figs/blank.pdf}
%   \end{minipage}
%   \begin{minipage}{0.45\textwidth}
%     \raggedleft
%     \includegraphics[width=1.0\linewidth]{figs/supervised_learning.pdf}
%     \caption{Supervised Task using Embeddings as Features}
%     \label{fig:figure2}
%   \end{minipage}
% \end{figure}


% Negative samples for contrastive learning are obtained via a corruption function $\mathcal{C}: \mathbb{R}^{N \times d} \times \mathbb{R}^{N \times N}  \rightarrow \mathbb{R}^{M \times d} \times \mathbb{R}^{M \times M}$, such that $\sampjointcorr{ij}=\mathcal{C}(\feat, \filter{i})$. The corruption function is designed in such a way that the data generated from the corruption function is decorrelated from the input data. Hence to learn representations across all filters in the filter bank, we maximize the average of the estimate of \mi~across all filters (considering $K$ filters):

To generate negative samples for contrastive learning, we employ a corruption function $\mathcal{C}: \mathbb{R}^{N \times d} \times \mathbb{R}^{N \times N} \rightarrow \mathbb{R}^{M \times d} \times \mathbb{R}^{M \times M}$, which yields corrupted samples denoted as $\sampjointcorr{ij}=\mathcal{C}(\feat, \filter{i})$. The designed corruption function generates data decorrelated with the input data. 

In order to learn representations across all filters in the filter bank, we aim to maximise the average estimate of mutual information (\mi) across all filters, considering $K$ filters.
\begin{equation}
    \mathcal{I}_{\filter{}} = \frac{1}{K}\sum_{i=1}^{K} \mathcal{I}^{JSD}_{i, \theta, \omega}(\featfilter{i}, \encproj{i})
\end{equation}
Maximising the Jenson-Shannon \mi~estimator is equivalent to reducing the binary cross entropy loss defined between positive samples (sampled from the joint) and the negative samples (sampled from the product of marginals). Therefore, for each filter, we minimise the following objective:
\begin{equation}
    \label{eq:loss_per_filter}
    \mathcal{L}_{\filter{i}} = \frac{1}{N + M}\left( \sum_{j=1}^{N}\mathbb{E}_{(\feat, \filter{i})}[\text{log}(D_{\omega}(h_{j}^{\filter{i}}, h_{g}^{\filter{i}}))] + \sum_{j=1}^{M}\mathbb{E}_{(\tilde{\feat}, \tilde{\filter{i})}}[\text{log}(1 - D_{\omega}(\tilde{h}_{j}^{\filter{i}}, h_{g}^{\filter{i}}))] \right)
\end{equation}
Therefore to learn meaningful representations across all filters the following objective is minimised:
\begin{equation}
    \label{eq:total_loss}
    \mathcal{L} = \frac{1}{K}\sum_{i=1}^{K} \mathcal{L}_{\filter{i}}
\end{equation}

However, managing the computational cost of training and storage for large graphs with separate node representations for each filter presents a significant challenge, exacerbated by the high dimensional requirements of contrastive learning methods. We implement parameter sharing to mitigate the first issue, borrowing the concept from studies such as \cite{gf:gprgnn, gf:bernnet}, thereby sharing the encoder's parameters $\theta$ and the discriminator's parameters $\omega$ across all filters. Instead of storing dense filter-specific node representations, we only store the parameters of the shared encoder and the first-hop neighbourhood information of each node per filter, which has a lower storage cost. For downstream tasks, we retrieve the embeddings by reconstructing filter-specific representations. To ensure quick and efficient reconstruction, we use a simple one-layer GNN. This on-demand reconstruction of filter-specific representations significantly reduces the computational and storage requirements associated with individual node representations. Fig~\ref{fig:unsup_learning} illustrates such a simple encoder's mutual information-based learning process.


Addressing the second issue, we initially train our models to generate low-dimensional embeddings. These encapsulate latent classes, as discussed in \cite{misc:latent_classes} as a superset of classes pertinent to downstream tasks. Although the low-dimensional embeddings harbour latent class information, they lack linear separability. Hence, we project these embeddings into a higher-dimensional space using random Fourier feature (RFF) projections, a strategy inspired by kernel methods (Section~\ref{subsec:random_feature_maps}). Using this approach allows for improved linear separability of the latent classes. Our experimental findings (Section~\ref{subsec:exp_rff_projections}) affirm the effectiveness of projecting lower-dimensional embeddings into higher dimensions, confirming the retention of latent class information in these embeddings.

%\begin{wrafigure}{r}{0.6\textwidth}
% \begin{figure}
%   \centering
%   %\includegraphics[width=\linewidth]{figs/supervised_learning.pdf}
%   \includegraphics[scale=0.32]{figs/supervised_learning.pdf}
%   \caption{Supervised Learning: Using the trained parameter $\Theta$, we generate the node embeddings by encoding the filtered graphs that get consumed in the classification task.}\label{fig:supervised}
%     \label{fig:sup_learning}
% \end{figure}
%\end{wrapfigure}

\subsection{Supervised Representation Learning}
\label{subsec:supervised_representation_learning}

% Once the representations per filter are obtained, one would need to learn a an aggregation mechanism to combine information from representations that represent different parts of the eigenspectrum, for the task at hand. We rely on learning schemes proposed in \cite{gf:gprgnn, gf:bernnet, gf:ppgnn}, where a weighted combination of filter specific representation is learnt. Hence, the combined representations we learn for the downstream task are as follows (for $K$ filters belonging to filter bank $\mathbf{F}$):
After obtaining representations for each filter post the reconstruction of the node representations, learning an aggregation mechanism to combine information from representations that capture different parts of the eigenspectrum for the given task is necessary. We adopt learning schemes proposed in \cite{gf:gprgnn, gf:bernnet, gf:ppgnn}, where we learn a weighted combination of filter-specific representations. Therefore, the combined representations we learn for the downstream task are as follows (considering $K$ filters from the filter bank $\mathbf{F}$):
\begin{equation}
    Z = \sum_{i=1}^{K}\alpha_{i}\phi'( \encproj{i})  
\end{equation}



The parameters $\alpha_{i}$'s are learnable. Additionally, the function $\phi(.)'$ represents either the \rff~projection or an identity transformation, depending on whether $\encproj{i}$ is low-dimensional or not. A classifier model (e.g. logistic regression) consumes these embeddings, where we train both the $\alpha_{i}$'s and the weights of the classifier. Fig \ref{fig:sup_learning} illustrates this process. The main distinction between semi-supervised methods such as \cite{gf:ppgnn, gf:gprgnn, gf:bernnet} and our method is that the semi-supervised methods learn both the encoder and the combination coefficients based on labelled data. However, we pre-train the encoder in our method and subsequently learn a task-specific combination of filter-specific representations.

\begin{figure}
  \centering
  %\includegraphics[width=\linewidth]{figs/supervised_learning.pdf}
  \includegraphics[scale=0.31]{figs/supervised_learning.pdf}
  \caption{Supervised Learning: Using the trained parameter $\Theta$, we generate the node embeddings by encoding the filtered graphs that get consumed in the classification task.}\label{fig:supervised}
    \label{fig:sup_learning}
\end{figure}


% While our approach would generate representations that capture the entire eigenspectrum, storing separate patch level representations (per filter) can become prohibitively expensive for large graphs. Moreover, generally, contrastive learning methods require higher dimensions, increasing both the computational cost of training as well as storage. To tackle the first issue, we share the parameters $\theta, \omega$ of the encoder and the discriminator respectively across all filters. This is inspired by works such as \cite{gf:gprgnn, gf:bernnet} where the encoder is shared across multiple filters. We believe that $\theta$ can be shared across all the encoders as each filter $\filter{i}$ projects the representations into its own corresponding Hilbert space in $\mathbb{R}^{d'}$. This allows us to reconstruct filter-specific representations as needed, while also reducing the computational and storage load. 

% To combat the second problem, we first train our models to generate very low dimensional embeddings. As discussed in \cite{misc:latent_classes}, there exist latent classes where each data point belongs to. These latent classes are defined to be a superset of set of classes defined for each downstream task. We believe that even for the current setting, these latent classes exist, and this notion of latent classes is also captured in lower dimensional embeddings. However, while these lower dimensional embeddings contain this latent class information, this information is no longer linearly separable. Hence, to achieve good downstream performance, we need to project these embeddings to a higher dimensional space (where these latent classes would be linearly separable). Inspired by kernel methods (see \ref{subsec:random_feature_maps}), we use \rff~projections to lift these low dimensional embeddings to higher dimensions, so that these representations become more amenable. We experimentally show (see \ref{subsec:exp_rff_projections}) that projecting lower dimensional embeddings into higher dimensions does give competitive performance, alluding to the fact that lower dimensional embeddings do indeed contain some notion of latent classes.


% Dealing with large graphs and the computational cost of training and storage can pose challenges when storing separate patch-level representations for each filter. Additionally, contrastive learning methods typically require higher dimensions, further increasing the computational burden.

% The first issue is tackled by adopting parameter sharing, specifically sharing the encoder's parameters $\theta$ and the discriminator's parameters $\omega$ across all filters, a strategy inspired by works such as \cite{gf:gprgnn, gf:bernnet}. Arguably, the viability of sharing $\theta$ across all encoders stems from each filter $\filter{i}$ projecting the representations into its corresponding Hilbert space in $\mathbb{R}^{d'}$. This parameter sharing facilitates the reconstruction of filter-specific representations on demand, significantly reducing the computational and storage requirements associated with individual patch-level representations.

% The second issue is approached by initially training our models to produce low-dimensional embeddings. As discussed in \cite{misc:latent_classes}, latent classes, defined as a superset of the classes relevant to downstream tasks, encompass each data point. It is hypothesized that such latent classes persist in our setting and are encapsulated within the lower-dimensional embeddings. Despite these embeddings containing latent class information, they are not linearly separable. To boost downstream performance, these embeddings need to be projected into a higher-dimensional space where the latent classes can be linearly separated. We utilize random Fourier feature (RFF) projections, inspired by kernel methods (refer to Section \ref{subsec:random_feature_maps}), to lift the low-dimensional embeddings into higher dimensions, thereby enhancing the separability of the latent classes. Our experimental results (see \ref{subsec:exp_rff_projections}) illustrate competitive performance when projecting lower-dimensional embeddings into higher dimensions, suggesting that these embeddings indeed retain latent class information.

% Note that $\alpha_{i}$'s are learnable parameters. Also note that $\phi(.)$ represents the \rff~projection or an identity transformation based on whether $\filter{i}X\Theta$ is low dimensional or not. These embeddings are then passed to a logistic regression model, where both $\alpha_{i}$'s and the weights of the logistic regression model are tuned. Note that, one could also perform an \rff~projection after combining all the embeddings, and we show such an ablation study in \ref{subsec:exp_pre_vs_post}. The key difference between semi-supervised methods such as \cite{gf:ppgnn, gf:gprgnn, gf:bernnet} and \ourmethod~is that the semi-supervised methods learn both the encoder and the combination coefficients given labels. However, we apriori learn the encoder, and then learn a task dependent combination of filter specific representations. 
